Integrated packing, placement, scheduling, and routing of personalized production: a pharmaceutical Industry 4.0 use-case with a planar transport system

The recent emergence of planar transport systems necessitates re-evaluation of Flexible Manufacturing Systems (FMS) to address the simultaneous scheduling of internal logistics and production operations. By operating on a tile-based planar grid, these systems allow independent movers full two-dimensional freedom, mitigating inefficiencies inherent to traditional sequential lines. This paper applies a planar FMS framework to a real-world use case in the pharmaceutical industry: the automated production of personalized drugs. Implementing this system requires solving optimization problems at both tactical and operational levels. The tactical level involves decisions regarding production line layout and the positioning of drug dispensers. A Mixed-Integer Quadratic Programming model is utilized for the packing problem to exploit drug co-occurrence patterns found in historical patient data. Subsequently, we solve the placement problem - a bi-level problem combining an assignment problem with Shortest Hamiltonian paths with neighborhoods - to arrange dispensers in a layout minimizing expected travel distances. The operational level is encountered daily, scheduling individual movers to process new orders as quickly as possible. This scheduling problem is formulated using Constraint Programming, modeling movers as reservoir resources to ensure order completeness, complemented by a routing phase using an iterative conflict-resolution mechanism and DAG-based reasoning to convert schedules into conflict-free paths. Evaluation using real-world prescription data for 40 drugs shows the framework scales efficiently across several layout topologies for up to 500 orders, with schedules that are highly effective and computationally tractable for daily operations.

==> figs/tables/definitions.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{p{2cm}p{4cm}p{8cm}}
        \toprule
        \textbf{Notation} & \textbf{Definition} & \textbf{Description} \\
        \midrule
        $M$ & Set of movers & Set of all movers in the system. \\
        
        $G$ & Set of drugs & Set of all drugs. \\
        
        $P$ & Set of patients & Set of all patients. \\
        
        $T$ & Set of all tasks & Set of all dispensing and interface tasks. \\
        
        $A$ & Set of all alternatives & Set of all alternatives of dispensing and interface tasks. Details in Section~\ref{sched:math:variables} \\
        
        $K$ & Set of all dispensers and interfaces & Set of all dispensing units and interfaces.\\
        
        $D \subseteq \mathcal{P}(K)$ & Set of all tiles & Set of all dispensaries and interfaces \\
        & & A tile is an interface or a set of dispensers residing at the same coordinates\\
        & & Example: $d_1 = \{\textsc{$k_1$}, \textsc{$k_4$}, \textsc{$k_7$}\}$ \\
        & & $D = \{\{\textsc{$k_1$}, \textsc{$k_4$}, \textsc{$k_7$}\}, \{\textsc{$k_2$}, \textsc{$k_5$}, \textsc{$k_6$}\}, \dots\}$. \\
        
        $T_p \subseteq T$ & Set of tasks for patient $p \in P$ & Tasks associated with a specific patient. Example: $T_1 = $ \\
        & & $\{\textsc{start}, \textsc{lisinopril}, \textsc{simvastatin}, \textsc{finish}\}$. \\
        
        $O_k \subseteq T$ & Set of tasks for dispenser $k \in K$ & Set of all tasks that a given dispenser could fulfill. \\
        
        $D_t \subseteq D$ & Set of tiles capable of fulfilling task $t \in T$ & Tiles outfitted with a dispenser able to perform a specific task. \\
        
        $I \subseteq D$ & Set of all interface tiles & Collection of all interface tiles in the system \\
        
        $\text{type}(t)$ & Type of task $t \in T$ & Type of task. Types outlined in Table~\ref{table:sched:task_types}.\\
        \bottomrule
    \end{tabular}
    \caption{Mathematical notation \& parameters.}
    \label{table:sched:defs}
\end{table}

==> figs/tables/routing_cmax_effect_d10_ext.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{c|c|c|c|c|c|c|c|c}
             \toprule
            \multirow{2}{*}{\shortstack{Mover\\count}} &
            \multicolumn{2}{c}{Square $C_{\max}$} &
            \multicolumn{2}{c}{Doubleline $C_{\max}$} &
            \multicolumn{2}{c}{Ring $C_{\max}$} &
            \multicolumn{2}{c}{Line $C_{\max}$} \\
            \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
             & Scheduling & Routing & Scheduling & Routing & Scheduling & Routing & Scheduling & Routing \\
            \midrule
            1 & 33427 & +0~(0.0\%) & 34506 & +0~(0.0\%) & 35056 & +0~(0.0\%) & 35233 & +0~(0.0\%) \\
            2 & 16722 & +7~(0.0\%) & 17295 & +22~(0.1\%) & 17556 & +14~(0.1\%) & 17663 & +28~(0.2\%) \\
            3 & 11163 & +11~(0.1\%) & 11524 & +21~(0.2\%) & 11782 & +35~(0.3\%) & 11788 & +31~(0.3\%) \\
            4 & 8373 & +10~(0.1\%) & 8638 & +21~(0.2\%) & 8806 & +29~(0.3\%) & 8875 & +38~(0.4\%) \\
            5 & 6700 & +14~(0.2\%) & 6943 & +23~(0.3\%) & 7091 & +30~(0.4\%) & 7131 & +39~(0.5\%) \\
            6 & 5602 & +17~(0.3\%) & 5822 & +27~(0.5\%) & 5947 & +41~(0.7\%) & 5992 & +54~(0.9\%) \\
            7 & 4808 & +17~(0.4\%) & 5030 & +24~(0.5\%) & 5092 & +48~(0.9\%) & 5151 & +75~(1.5\%) \\
            8 & 4224 & +24~(0.6\%) & 4399 & +37~(0.8\%) & 4512 & +46~(1.0\%) & 4560 & +53~(1.2\%) \\
            9 & 3762 & +17~(0.5\%) & 3961 & +33~(0.8\%) & 4012 & +58~(1.4\%) & 4137 & +72~(1.7\%) \\
            10 & 3388 & +19~(0.6\%) & 3557 & +31~(0.9\%) & 3623 & +73~(2.0\%) & 3757 & +71~(1.9\%) \\
            11 & 3137 & +33~(1.1\%) & 3310 & +50~(1.5\%) & 3372 & +80~(2.4\%) & 3659 & +104~(2.8\%) \\
            12 & 2942 & +23~(0.8\%) & 3042 & +42~(1.4\%) & 3108 & +56~(1.8\%) & 3286 & +100~(3.0\%) \\
            \bottomrule
        \end{tabular}
    }
    \caption{Makespan values for different movers, before and after routing.}
    % \tn{jeste se da ten post-route napsat jen jako $+xx$ čimž se ušetří tak 2 číslice $\xrightarrow{}$ bude to užší}
    \label{table:expRouting:cmax_d10}
\end{table}

==> figs/tables/routing_cmax_effect_d1_ext.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{c|c|c|c|c|c|c|c|c}
            \toprule
            \multirow{2}{*}{\shortstack{Mover\\count}} &
            \multicolumn{2}{c}{Square $C_{\max}$} &
            \multicolumn{2}{c}{Doubleline $C_{\max}$} &
            \multicolumn{2}{c}{Ring $C_{\max}$} &
            \multicolumn{2}{c}{Line $C_{\max}$} \\
            \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
             & Scheduling & Routing & Scheduling & Routing & Scheduling & Routing & Scheduling & Routing \\
            \midrule
            1 & 4731 & +0~(0.0\%) & 5731 & +0~(0.0\%) & 6202 & +0~(0.0\%) & 6201 & +0~(0.0\%) \\
            2 & 2386 & +5~(0.2\%) & 2897 & +10~(0.3\%) & 3181 & +13~(0.4\%) & 3296 & +14~(0.4\%) \\
            3 & 1592 & +9~(0.6\%) & 1980 & +21~(1.1\%) & 2171 & +25~(1.2\%) & 2167 & +32~(1.5\%) \\
            4 & 1199 & +10~(0.8\%) & 1492 & +23~(1.5\%) & 1714 & +42~(2.5\%) & 1638 & +50~(3.1\%) \\
            5 & 962 & +16~(1.7\%) & 1187 & +33~(2.8\%) & 1362 & +27~(2.0\%) & 1410 & +32~(2.3\%) \\
            6 & 817 & +22~(2.7\%) & 1012 & +43~(4.2\%) & 1131 & +42~(3.7\%) & 1158 & +45~(3.9\%) \\
            7 & 710 & +22~(3.1\%) & 935 & +36~(3.9\%) & 969 & +46~(4.7\%) & 987 & +44~(4.5\%) \\
            8 & 619 & +23~(3.7\%) & 858 & +39~(4.5\%) & 914 & +52~(5.7\%) & 980 & +53~(5.4\%) \\
            9 & 571 & +23~(4.0\%) & 728 & +48~(6.6\%) & 813 & +46~(5.7\%) & 885 & +66~(7.5\%) \\
            10 & 524 & +24~(4.6\%) & 720 & +50~(6.9\%) & 743 & +41~(5.5\%) & 834 & +69~(8.3\%) \\
            11 & 500 & +34~(6.8\%) & 642 & +58~(9.0\%) & 712 & +43~(6.0\%) & 807 & +107~(13.3\%) \\
            12 & 448 & +37~(8.3\%) & 605 & +56~(9.3\%) & 665 & +60~(9.0\%) & 689 & +79~(11.5\%) \\
            \bottomrule
        \end{tabular} 
    }
    \caption{Makespan values for different movers, before and after routing with $10\times$ faster dispensing speed.}
    \label{table:expRouting:cmax_d1}
\end{table}


==> figs/tables/task_types.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{p{3cm}p{11cm}}
        \toprule
        \textbf{Task Type} & \textbf{Description} \\
        \midrule
        $\textsc{start}$ & Process of dropping a new capsule tray with empty capsules upon a mover, takes $\trayOperation$ time units. \\
        $\textsc{dispensing}$ & Process of dispensing of a dose of drug $g\in\drugs$ into each capsule on a capsule tray. \\
        $\textsc{finish}$ & Process of collecting a completed capsule tray, takes $\trayOperation$ time units. \\
        \bottomrule
    \end{tabular}
    \caption{Types of patient tasks. - \textbf{TN: kandidat}}
    \label{table:sched:task_types}
\end{table}

==> figs/topologies.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.33\textwidth}
      \centering
        \input{figs/square8x8}
      \caption{Square $8\times8/4$ topology.}
      \label{fig:optim_interface_locations:s8x8}
    \end{subfigure}%
    \begin{subfigure}[t]{0.33\textwidth}
      \centering
          \input{figs/square7x7}
      \caption{Square $7\times7/2$ topology.}
      \label{fig:optim_interface_locations:s7x7}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
      \centering
          \input{figs/square6x6}
      \caption{Square $6\times6/1$ topology.}
      \label{fig:optim_interface_locations:s6x6}
    \end{subfigure}

    \vspace{1em}

    \begin{subfigure}[t]{0.33\textwidth}
      \centering
         \input{figs/ring64}
      \caption{Ring $64/4$ topology.}
      \label{fig:optim_interface_locations:r68}
    \end{subfigure}%
     \begin{subfigure}[t]{0.63\textwidth}
      \centering
        \input{figs/doubleline48}
      \caption{Doubleline $50/2$ topology.}
      \label{fig:optim_interface_locations:d50}
    \end{subfigure}%

    
    \caption{Optimized locations of interfaces in different topologies.}
    \label{fig:optim_interface_locations}
\end{figure}

==> notations.tex <==
% Add this line to the preamble of your main .tex file,
% before the notation preamble.
\usepackage{xcolor}
\usepackage{xspace}

% ======================================================================
% STRT OF NOTATION PREAMBLE
% ======================================================================

% --- 1. General & High-Level Sets ---
\newcommand{\patientsHistory}{\ensuremath{\textcolor{red}{\mathcal{P}_{\text{history}}}}\xspace}
\newcommand{\patients}{\ensuremath{\textcolor{red}{\mathcal{P}}}\xspace}
\newcommand{\layout}{\ensuremath{\textcolor{red}{\mathcal{H}}}\xspace}
\newcommand{\interfaces}{\ensuremath{\textcolor{red}{\mathcal{I}}}\xspace}
\newcommand{\movers}{\ensuremath{\textcolor{red}{\mathcal{M}}}\xspace}
\newcommand{\tiles}{\ensuremath{\textcolor{red}{\mathcal{K}}}\xspace}
\newcommand{\drugs}{\ensuremath{\textcolor{red}{\mathcal{G}}}\xspace}

% --- 2. Packing & Placement Problem Variables ---
\newcommand{\numTiles}{\ensuremath{\textcolor{red}{n_{\text{tiles}}}}\xspace}
\newcommand{\numMovers}{\ensuremath{\textcolor{red}{n_{\text{movers}}}}\xspace}
\newcommand{\numDispensers}{\ensuremath{\textcolor{red}{n_{\text{dispensers}}}}\xspace}
\newcommand{\packing}{\ensuremath{\textcolor{red}{\mathcal{U}}}\xspace}
\newcommand{\drugUtil}{\ensuremath{\textcolor{red}{u_i}}\xspace}
\newcommand{\dispenserCount}{\ensuremath{\textcolor{red}{z_i}}\xspace}
\newcommand{\dispenserLoad}{\ensuremath{\textcolor{red}{\pi_i}}\xspace}
\newcommand{\tileLoad}{\ensuremath{\textcolor{red}{\mu_k}}\xspace}
\newcommand{\maxTileLoad}{\ensuremath{\textcolor{red}{\mu_{\max}}}\xspace}
\newcommand{\hatMaxLoad}{\ensuremath{\textcolor{red}{\hat{\mu}_{\max}}}\xspace}
\newcommand{\hatDispenserCount}[1][i]{\ensuremath{\textcolor{red}{\hat{z}_#1}}\xspace}
\newcommand{\hatDispenserLoad}{\ensuremath{\textcolor{red}{\hat{\pi}_i}}\xspace}
\newcommand{\placement}{\ensuremath{\textcolor{red}{g}}\xspace}
\newcommand{\placementExt}{\ensuremath{\textcolor{red}{g: \tiles \mapsto \layout}}\xspace}
\newcommand{\permElement}[1][]{\ensuremath{\textcolor{red}{\sigma_{#1}}}\xspace}
\newcommand{\tilesDistance}[1]{\ensuremath{\textcolor{red}{\| \placement(\permElement_#1) - \placement(\permElement_{#1+1}) \|_1}}\xspace}

% --- 3. Scheduling Problem Variables ---
\newcommand{\distMatrix}{\ensuremath{\textcolor{red}{\mathcal{L_{\tiles}}}}\xspace}
\newcommand{\schedule}{\ensuremath{\textcolor{red}{s}}\xspace}
\newcommand{\tasks}{\ensuremath{\textcolor{red}{\mathcal{T}}}\xspace}
\newcommand{\sites}{\ensuremath{\textcolor{red}{\mathcal{V}}}\xspace}
\newcommand{\transits}{\ensuremath{\textcolor{red}{\mathcal{W}}}\xspace}
\newcommand{\taskAlternatives}{\ensuremath{\textcolor{red}{\mathcal{A}}}\xspace}
\newcommand{\dispensingUnits}{\ensuremath{\textcolor{red}{\mathcal{K}}}\xspace}
\newcommand{\tasksForPatient}[1]{\ensuremath{\textcolor{red}{\mathcal{S}_{#1}}}\xspace}
\newcommand{\tasksForDispenser}[1]{\ensuremath{\textcolor{red}{\mathcal{O}_{#1}}}\xspace}
\newcommand{\trayOperation}{\ensuremath{\textcolor{red}{\eta^{\interfaces}}}\xspace}
\newcommand{\shortestPathPatient}{\ensuremath{\textcolor{red}{\kappa_p}}\xspace}
\newcommand{\patientPathTime}[1][p]{\ensuremath{\textcolor{red}{\eta^\prime_{#1}}}\xspace}


% --- 4. Helper Functions & Operators ---
\newcommand{\tilesForDrug}[1]{\ensuremath{\textcolor{red}{\mathcal{D}_{#1}}}\xspace}
\newcommand{\dispensersOnTile}[1]{\ensuremath{\textcolor{red}{\text{Dispensers}(#1)}}\xspace}

% ======================================================================
% END OF NOTATION PREAMBLE
% ======================================================================
